Graph Reparameterizations for Enabling 1000+ Monte Carlo Iterations in Bayesian Deep Neural Networks

Uncertainty estimation in deep models is essential in many real-world applications and has benefited from developments over the last several years. Recent evidence suggests that existing solutions dependent on simple Gaussian formulations may not be sufficient. However, moving to other distributions necessitates Monte Carlo (MC) sampling to estimate quantities such as the KL divergence: it could be expensive and scales poorly as the dimensions of both the input data and the model grow. This is directly related to the structure of the computation graph, which can grow linearly as a function of the number of MC samples needed. Here, we construct a framework to describe these computation graphs, and identify probability families where the graph size can be independent or only weakly dependent on the number of MC samples. These families correspond directly to large classes of distributions. Empirically, we can run a much larger number of iterations for MC approximations for larger architectures used in computer vision with gains in performance measured in confident accuracy, stability of training, memory and training time.

==> impacts.tex <==
\section*{Ethical Impact}



Our research contributes to the general area dealing with the development and deployment of Bayesian Deep Neural Networks, providing a practical approach with statistical justification to efficiently increase number of MC samples when training on GPUs with limited memory. This enables decreasing training variance and offers 
improvements in the model's performance. The research should be able to benefit efforts focused on applications of Bayesian deep neural networks for real world problems, where an incorrect prediction from the model can have undesirable consequences. Autonomous vehicles, financial markets, and healthcare are some examples. 

Endowing systems with predictive uncertainty has the potential to improve and enable automation across all types of fields. With large amounts of data, applications such as clinical diagnosis may benefit significantly from accurate, confident predictions based on models learned from millions of other patients.
Our work may slightly disadvantage individuals with specific job 
profiles that will suffer due to automation,
but is a problem that needs to be addressed at a legislative or societal level.

While our work does not directly negatively impact specific groups of individuals, it could be the case that too much reliance on automated method without corroboration or quality control procedures could lead to incorrect judgments which would have otherwise been avoided.

While we do not believe that our model explicitly leverages biases within the data, indirectly, confidence learned by our model \textit{could} be correlated with protected/sensitive features or subsets of the input, leading to bias (high accuracy on high confidence sets correlated with $X$, while 
$\neg X$ suffer due to low confidence).







